Mono-SF: Multi-View Geometry Meets Single-View Depth for Monocular Scene Flow Estimation of Dynamic Traffic Scenes

Existing 3D scene flow estimation methods provide the 3D geometry and 3D motion of a scene and gain a lot of interest, for example in the context of autonomous driving. These methods are traditionally based on a temporal series of stereo images. In this paper, we propose a novel monocular 3D scene flow estimation method, called Mono-SF. Mono-SF jointly estimates the 3D structure and motion of the scene by combining multi-view geometry and single-view depth information. Mono-SF considers that the scene flow should be consistent in terms of warping the reference image in the consecutive image based on the principles of multi-view geometry. For integrating single-view depth in a statistical manner, a convolutional neural network, called ProbDepthNet, is proposed. ProbDepthNet estimates pixel-wise depth distributions from a single image rather than single depth values. Additionally, as part of ProbDepthNet, a novel recalibration technique for regression problems is proposed to ensure well-calibrated distributions. Our experiments show that Mono-SF outperforms state-of-the-art monocular baselines and ablation studies support the Mono-SF approach and ProbDepthNet design.

==> tables/Experiments/ProbDepthNetKittiEigen.tex <==
\begin{table*}[tbhp]
\centering
\setlength\tabcolsep{2 pt}
\begin{tabular}{>{\centering}m{4.2cm} || c || c c c c | c c c}
\multirow{2}{*}{Method} & \multirow{2}{*}{Cap} & \multicolumn{4}{c|}{lower is better} &  \multicolumn{3}{c}{higher is better} \\ 
& & Abs Rel & Sq Rel & RMSE & $\text{RMSE}_{log}$ & $\delta < 1.25$ & $\delta < 1.25^2$ & $\delta < 1.25^3$  \\ \hline \hline
Eigen et al. \cite{eigen2014depth} & 0 - 80 m & 0.190 & 1.515 & 7.156 & 0.270 & 0.692 & 0.899 & 0.967 \\
Liu et al. \cite{liu2016learning} & 0 - 80 m & 0.217 & 1.841 & 6.986 & 0.289 &0.647 & 0.882 & 0.961 \\
LRC \cite{godard2016deepdepth} & 0 - 80 m & 0.114 & 0.898 & 4.935 & 0.206 & 0.861 & 0.949 & 0.976 \\ 
Kuznietsov et al. \cite{kuznietsov2017semi} & 0 - 80 m & 0.113 & 0.741 & 4.621 & 0.189 & 0.862 & 0.960 & 0.986 \\
DORN \cite{fu2018deep} & 0 - 80 m & 0.111 & 0.618 & 3.659 & 0.168& 0.894 & 0.964 & 0.984 \\
ProbDepthNet & 0 - 80 m & 0.103 & 0.762 & 4.680 & 0.195 & 0.871 & 0.953 & 0.979 \\ \hline
Garg et al. \cite{garg2016singleviewdepth} & 0 - 50 m & 0.169 & 1.080 & 5.104 & 0.273 & 0.740 & 0.904 & 0.962 \\
LRC \cite{godard2016deepdepth} & 0 - 50 m & 0.108 & 0.657 & 3.729 & 0.194 & 0.873 & 0.954 & 0.979 \\
Kuznietsov et al. \cite{kuznietsov2017semi} & 0 - 50 m & 0.108 & 0.595 & 3.518 & 0.179 & 0.875 & 0.964 & 0.988 \\
DORN \cite{fu2018deep} & 0 - 50 m & 0.108 & 0.535 & 2.884 & 0.162 & 0.902 & 0.966 & 0.985 \\
ProbDepthNet & 0 - 50 m & 0.098 & 0.567 & 3.530 & 0.183 & 0.883 & 0.959 & 0.981 \\ \hline \hline
\multicolumn{9}{l}{\footnotesize \textit{ \textbf{Abs Rel}, \textbf{Sq Rel}: absolute and squared relative depth error; \textbf{RMSE}: root mean squared depth error }} \\
\multicolumn{9}{l}{\footnotesize \textit{ \textbf{$\text{RMSE}_{log}$}: root mean squared logarithmic depth error; $\boldsymbol{\delta < 1.25^k}$: frequency of predictions fulfilling a quality threshold }}
\end{tabular}
\caption{Quantitative evaluation of methods for single-view depth prediction on the KITTI dataset \cite{Geiger2013IJRR} using the test split by Eigen et al. \cite{eigen2014depth}.}
\label{tab_ProbDepthNetKittiEigen}
\end{table*}
